Fast exact algorithms via the Matrix Tree Theorem

Fast exact algorithms are known for Hamiltonian paths in undirected and directed bipartite graphs through elegant though involved algorithms that are quite different from each other. We devise algorithms that are simple and similar to each other while having the same upper bounds. The common features of these algorithms is the use of the Matrix-Tree theorem and sieving using roots of unity. Next, we use the framework to provide alternative algorithms to count perfect matchings in bipartite graphs on $n$ vertices, i.e., computing the $\{0,1\}$-permanent of a square $n/2 \times n/2$ matrix which runs in a time similar to Ryser. We demonstrate the flexibility of our method by counting the number of ways to vertex partition the graph into $k$-stars (a $k$-star consist of a tree with a root having $k-1$ children that are all leaves). Interestingly, our running time improves to $O^*((1+\epsilon_k)^n)$ with $\epsilon_k \rightarrow 0$ as $k \rightarrow \infty$. As an aside, making use of Bj\"orklund's algorithm for exact counting perfect matchings in general graphs, we show that the count of maximum matchings can be computed in time $O^*(2^\nu)$ where $\nu$ is the size of a maximum matching. The crucial ingredient here is the famous Gallai-Edmonds decomposition theorem. All our algorithms run in polynomial space.

==> bipHam.tex <==
\section{Hamiltonian Paths in Bipartite Graphs}
\subsection{Undirected} Let $G=(V_1\sqcup V_2, E)$ be an undirected bipartite graph, with $|V_1|=|V_2|+1 = n$. Let $s$ and $t$ be two distinct vertices in $V_1$. From $G$ we define an undirected multi-graph, $G_1 = (V_1,E_1)$ on vertices in $V_1$, as follows. There is an edge $\{u,v\}$ in $G_1$ labelled $w$, denoted $(\{u,v\},w)$, if and only if $u,v\in V_1, w\in V_2$ and $\{u,w\},\{w,v\}\in E$. Let $B(G_1)$ be the incidence matrix of $G_1$ (arbitrarily oriented). Let $B^s(G_1)$ be $B(G_1)$ once row $s$ has been removed from it. Let $\mcX=\{x_e|e\in E_1\}$ be a set of indeterminates. Let $B^s(G_1,\mcX)$ be defined as before. 

We define another rectangular matrix $C$, of dimension $(n-1)\times |E_1|$ as follows. Its rows are indexed by the vertices in $V_2$ and the columns are indexed by the edges in $E_1$ (in the same order as in $B^s(G_1)$). The entry in the row $q$ (a vertex in $V_2$) and column $e$ is as follows. 
	\[
		C[q,e (=(\{u,v\},w))] = 
		\left\{
		\begin{array}{ll}
			1 & \mbox{ if } q=w\\
			0 & \mbox{ otherwise.} 
		\end{array}
		\right.
	\] 
Consider the following polynomial in $\mcX$ variables.
\[
	h(\bold{x}) = \det\left(B^s(G_1,\mcX)C^{\top}\right)
\]
Let $\mathcal{Z}=\{z_u|u\in V_1\}$ be a set of indeterminates and $y$ be another indeterminate. Consider substituting for each $x_e$, ($e= (\{u,v\}w)$), $y^{k(e)}z_uz_v$, in $h(\bold{x})$ where $k(e)$ is number from $[2n^3]$ chosen uniformly at random. Let the resulting polynomial be $g(\bold{z},y)$. That is,
\[
	g(\bold{z},y) = \det\left(B^s(G_1,\mcX)C^{\top}\right)\big\vert_{x_e = y^{k(e)}z_uz_v; ~e= (\{u,v\},w), ~k(e)\in_r[2n^3]}.
\]   
\begin{lemma}
	If there exists a $st$-hamitonian path in $G$, then with probability at least $1/2$ 
	\[
		\sum_{\bold{z}\in \sU_2^{n}}^{}z_sz_tg(\bold{z},y) \neq 0.
	\] 
	Otherwise, the left hand side above is equal to zero. 
\end{lemma}
\begin{proof}
	Using~\cref{thm:CBT} we can write,
	\[
		\det\left(B^s(G_1,\mcX)C^{\top}\right) = \sum_{S\subseteq E_1,|S|=n-1}^{}\det(B^s(G_1,\mcX)[S])\det(C^\top[S]).
	\]
	Clearly, $S\subseteq E_1$ of size $n-1$ contributes to the sum on the right hand side above, if and only if both $\det(B^s(G_1,\mcX)[S])$ and $\det(C^\top[S])$ are non-zero. Which means, $S$ should form a spanning tree of $G_1$ and that each vertex from $V_2$ appears exactly once as label of some edge in $S$. So, in the case when both are non-zero, we get a non-zero monomial $\sigma\prod_{e\in S}^{}x_e$, where $\sigma\in\{-1,1\}$. 
	If, additionally, $S$ in right hand side, corresponds to a $st$-hamiltonian path in $G_1$ then we can say that there is a $st$-hamiltonian path in $G$. Similar to the proof of~\cref{lem:dham}, we can see that $S$ corresponds to a hamiltonian path in $G_1$ if and only if the corresponding monomial (in $z_sz_tg(\bold{z},y)$ obtained after the substitution $x_e= y^{k(e)}z_uz_v$ for $e = (\{u,v\},w)$ in $h(\bold{x})$) is $\prod_{u\in V_1}z^2_u$. The $y^{k(e)}$ is used to ensure that, w.h.p., there is unique monomial (in $\mathcal{Z}$ variables) of the desired form with the least possible exponent of $y$, using isolation lemma. 
\end{proof} 

\subsection{Directed} Now, we consider a directed bipartite graph $G=(V_1\sqcup V_2,E)$, with $|V_1|=|V_2|+1=n$. Let $s$ and $t$ be two distinct vertices in $V_1$. We define from $G$ a directed multi-graph $G_1 = (V_1,E_1)$ on vertices in $V_1$ as follows. There is an edge $uv$ in $G_1$ labelled $w$, denoted $(uv,w)$, if and only if $u,v\in V_1,w\in V_2$ and $uw,wv\in E$. Let $B(G_1)$, $B^s(G_1)$ and $B^s(G_1,\mcX)$ be defined as usual. Let $C$, a matrix of dimension $(n-1)\times |E_1|$ be defined similar to the undirected bipartite graphs case. 
Let $h(\bold{x})$ be defined as earlier. Consider substituting for each $x_e$ ($e = (uv,w)$), $y^{k(e)}z^2_uz_v$ in $h(\bold{x})$, where $k(e)$ is a number from $[2n^3]$ chosen uniformly at random. Let the resulting polynomial be $g(\bold{z},y)$. That is,
\[
	g(\bold{z},y) = \det\left(B^s(G_1,\mcX)C^{\top}\right)\big\vert_{x_e = y^{k(e)}z^2_uz_v; ~e= (uv,w), ~k(e)\in_r[2n^3]}.
\]
\begin{lemma}
	If there is a directed $st$-hamiltonian path in $G$, then with probability at least $1/2$
	\[
		\sum_{\bold{z}\in \sU_3^{n}}^{}z_sz^2_tg(\bold{z},y) \neq 0
	\] 
	where $\sU_3=\{1,\omega,\omega^2\}$ and $\omega$ is the cube root of unity.
	Otherwise, the left hand side above is equal to zero.
\end{lemma}
\begin{proof}
	Again, using the~\cref{thm:CBT} we can write,
	\begin{equation}
		\label{eq:dirCBT}
		\det\left(B^s(G_1,\mcX)C^{\top}\right) = \sum_{S\subseteq E_1,|S|=n-1}^{}\det(B^s(G_1,\mcX)[S])\det(C^\top[S]).
	\end{equation}
	So, $S\subseteq E_1, |S| = n-1$ in the right hand side above contributes non-zero term if and only if both the determinants on the right hand side are non-zero, i.e., $S$ forms a spanning tree (of the underlying undirected graph) and every vertex from $V_2$ appears exactly once as a label of some edge in $S$. 
	
	It is clear that, if the spanning tree corresponding to $S$ is actually a directed $st$-hamiltonian path then it contributes the monomial $\prod_{u\in V_1}z^3_u$ in $(z_sz^2_tg(\bold{z},y))$. In general, the $\prod_{e\in S}x_e$ is present in the right hand side summation in ~\cref{eq:dirCBT}. After the substitution $x_e= y^{k(e)}z^2_uz_v; e=(uv,w),k(e)\in_r[2n^3]$, in $h(\bold{x})$, to get $z_sz^2_tg(\bold{z},y)$, each edge in $S$ contributes a degree $3$ to the monomial. If the spanning tree is not a (directed or undirected )$st$-hamiltonian path then there is a leaf node $v\neq t$ in $S$, and the corresponding edge either contributes $z_v$ or $z^2_v$ (if the edge directed towards $v$ or away from $v$ respectively). Such monomials get cancelled with each other over the sum on $\bold{z}\in\{1,\omega,\omega^2\}^n$. If the spanning tree $S$ is an undirected $st$-hamiltonian path but not a directed $st$-hamiltonian path then there exists a node $v$ that contributes $z^2_v$ or $z^4_v$, both of which ensure that the corresponding monomials get cancelled with each other over the sum $\bold{z}\in\{1,\omega,\omega^2\}^n$. 
	
	So, only if the underlying spanning tree $S$ is a directed $st$-hamiltonian path, the corresponding monomial survives the summation over the cube roots of unity. However, to avoid cancellation with hamiltonian paths with opposite sign, we use the fact that with high probability one will survive due to isolation lemma.             
\end{proof}   

  

==> forests.tex <==


%\begin{comment}
	\subsection{Directed}
	Let $G=(V,E)$ be a directed graph with $|V|=n,|E|=m$. Define its edge-incidence matrix $B\in \bbZ_2^{n\times m}$ and indegree matrix $B_{in}'$ as follows:
	
	\begin{minipage}{.4\textwidth}
		\[ B[v,e=(u,w)]=\begin{cases} 
			1 & v=u \\
			-1 & v=w\\
			0 & \text{otherwise} 
		\end{cases}
		\]
	\end{minipage}% This must go next to `\end{minipage}`
	\begin{minipage}{.5\textwidth}
	\[ B_{in}'[v,e=(u,w)]=\begin{cases} 
		1 & v=w \\
		0 & \text{otherwise} 
	\end{cases}
	\]
	\end{minipage}
	
	Denote by $B_x$ the matrix where the $e_{th}$ column of $U$ is multiplied by the variable $x_e$. Let $y$ be a variable. Let $B_{x,y}$ and $B_{in}$ be the matrices
	
	\begin{minipage}{.4\textwidth}
	\[
	B_{x,y} = \left[\begin{array}{ c | c }
		B_x & y I_{n\times n} 
	\end{array}\right]
	\]
	\end{minipage}% This must go next to `\end{minipage}`
\begin{minipage}{.5\textwidth}
\[
B_{in} = \left[\begin{array}{ c | c }
B_{in}' &  I_{n\times n} 
\end{array}\right]
\]
\end{minipage} 
\begin{definition}
An Arborescence Cover of $G$ is a set of arborescences that cover all the vertices of $G$. A $k$-arborescence cover of $G$ is a arborescence cover of $G$ consisting of $k$ arborescences. We call a arborescence cover to be $S$-rooted if the set of roots of the arborescences contains $S$ as a subset.
\end{definition}
\begin{theorem}
For any $k\le n$, $[y^k]\det(B_{x,y}B_{in}^\top)$ is the polynomial of rooted $k$-arborescence covers of $G$. Moreover, for $S\subseteq V$, $[y^k]\det(B_{x,y}(S)B_{in}^\top(S))$ is the polynomial of $S$-rooted $(|S|+k)$-arborescence covers of $G$.
\end{theorem}


%\end{comment}

